Synthesis of sup-interpretations: a survey

In this paper, we survey the complexity of distinct methods that allow the programmer to synthesize a sup-interpretation, a function providing an upper- bound on the size of the output values computed by a program. It consists in a static space analysis tool without consideration of the time consumption. Although clearly related, sup-interpretation is independent from termination since it only provides an upper bound on the terminating computations. First, we study some undecidable properties of sup-interpretations from a theoretical point of view. Next, we fix term rewriting systems as our computational model and we show that a sup-interpretation can be obtained through the use of a well-known termination technique, the polynomial interpretations. The drawback is that such a method only applies to total functions (strongly normalizing programs). To overcome this problem we also study sup-interpretations through the notion of quasi-interpretation. Quasi-interpretations also suffer from a drawback that lies in the subterm property. This property drastically restricts the shape of the considered functions. Again we overcome this problem by introducing a new notion of interpretations mainly based on the dependency pairs method. We study the decidability and complexity of the sup-interpretation synthesis problem for all these three tools over sets of polynomials. Finally, we take benefit of some previous works on termination and runtime complexity to infer sup-interpretations.

==> macroSI.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bon � r�fl�chir sur la notation
\newcommand{\q}{\mbox{\textbf{q}}}
% � remplacer par expression
\edef\termone{t}
\edef\termtwo{u}
\edef\termthree{v}
\edef\termfour{w}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% les classiques

\newcommand{\tsome}[3]{\theta(#1_{#2}\sigma), \cdots, \theta(#1_{#3}\sigma)}
\newcommand{\tmany}[2]{\tsome{#1}{1}{#2}}
\newcommand{\ttsome}[3]{\theta(#1_{#2}), \cdots, \theta(#1_{#3})}
\newcommand{\ttmany}[2]{\ttsome{#1}{1}{#2}}
\newcommand{\ataillesome}[3]{\alpha\taille{#1_{#2}}, \cdots, \alpha\taille{#1_{#3}}}
\newcommand{\ataillemany}[2]{\ataillesome{#1}{1}{#2}}
\newcommand{\height}[1]{h(#1)}
\newcommand{\NPtime}{\mbox{\sc NPtime}}

\newcommand{\Ptime}{\mathsf{P}}
\newcommand{\bQ}{\mathbb{Q}^+}
\newcommand{\inter}[1]{\llceil #1 \rrceil}
\newcommand{\id}{\texttt{id}}
\newcommand{\funfive}{\texttt{h}}
\def\funsix{\mbox{\texttt{s}}}




% Sup interpretation


%Equations

%Op�rateurs en bf

% If then else
%\newcommand{\Si}[3]{\mathbf{If\ }#1\mathbf{\ Then\ }#2\mathbf{\ Else\ }#3}

% definition par cas
\newcommand{\Cas}[1]{
\begin{array}{ll}
\mathbf{Case\ }  #1\mathbf{\ of\ } & \\
&
\begin{array}{ll}
\patone_1 & \rightarrow #1_1 \\
\ldots \\
\patone_\ell & \rightarrow #1_\ell 
\end{array}
\end{array}
}

\newcommand{\CasPlat}[1]{
\mathbf{Case\ }  #1\mathbf{\ of\ } 
\patone_1 \rightarrow #1_1 
\ldots 
\patone_\ell \rightarrow #1_\ell 
}

\newcommand{\CasPlats}[1]{
\mathbf{Case\ }  \overline{#1 } \mathbf{\ of\ } 
\overline{\patone_1} \rightarrow #1_1 
\ldots 
\overline{\patone_\ell} \rightarrow #1_\ell 
}

\newcommand{\CasPlatss}[1]{
\mathbf{Case\ }  \overline{#1 } \mathbf{\ of\ } 
\overline{\patone_1} \rightarrow e_1 
\ldots 
\overline{\patone_\ell} \rightarrow e_\ell 
}

\newcommand{\CasPlate}[1]{
\mathbf{Case\ }  #1\mathbf{\ of\ } 
\sone_1 \rightarrow #1_1 
\ldots 
\sone_\ell \rightarrow #1_\ell 
}
% Constructeurs en bf
%\newcommand{\Values}{\mathit{Values}}











\edef\termone{t}
\edef\termthree{v}
\edef\termfour{w}

\def\reftransto{\mbox{${\stackrel{*\;}{\to}}$}}



\newcommand{\size}{\mbox{\texttt{size}}}
\newcommand{\concat}{\mbox{\emph{\texttt{shuffle}}}}
%\newcommand{\pol}{\texttt{pol}}
\newcommand{\match}{\mbox{\texttt{match}}}
\newcommand{\et}{\mbox{\texttt{and}}}
\newcommand{\equivFdeux}{\approx_{ \Functions_2}}
\newcommand{\precFdeux}{\geq_{ \Functions_2}}
\newcommand{\ConstermsU}{\Terms{\Constructors_1 \cup \Constructors_2}}

\newcommand{\fn}[2]{ \lambda #1. #2}
\def\coef{\mbox{\texttt{coef}}}
\newcommand{\TermsU}{\Terms{\Constructors_1 \cup \Constructors_2,\Functions_1 \cup \Functions_2,\Variables_1 \cup \Variables_2}}
\newcommand{\progj}{\langle \Variables_j, \Constructors_j, \Functions_j,
         \Equations_j \rangle}
         
\newcommand{\MaxPlus}{\mathsf{MaxPlus}}
\newcommand{\MaxPoly}{\mathsf{MaxPoly}}
\newcommand{\kdMaxPoly}{{\mathsf{MaxPoly}}^{(\mathsf{k},\mathsf{d})}}
\newcommand{\kdMaxPlus}{{\mathsf{MaxPlus}}^{(\mathsf{k},\mathsf{d})}} 
\newcommand{\kdmMaxPoly}{{\mathsf{MaxPlus}}^{(\mathsf{k}^{\taille{t}},\mathsf{d}^{\taille{t}})}}

      



\def\skop{\texttt{skip}}
\def\return{\texttt{return}}
\def\command{\texttt{Cm}}
\def\class{\texttt{C}}
\def\Class{\texttt{Class}}
\def\main{\texttt{main}}
\def\decla{\texttt{D}}
\def\varcom{\texttt{K}}

\def\move{\mbox{\texttt{move}}}
\def\position{\mbox{\texttt{Coord}}}
\def\transition{\mbox{\texttt{transition}}}
\newcommand{\Parameters}{\mathcal{P}}  
 \def\op{\mathbf{op}}
 \edef\attribut{A}
\edef\Attribut{A}
\newcommand{\new}{\texttt{new} \ }
       
